Benchmarking Specialized Databases for High-frequency Data

This paper presents a benchmarking suite designed for the evaluation and comparison of time series databases for high-frequency data, with a focus on financial applications. The proposed suite comprises of four specialized databases: ClickHouse, InfluxDB, kdb+ and TimescaleDB. The results from the suite demonstrate that kdb+ has the highest performance amongst the tested databases, while also highlighting the strengths and weaknesses of each of the databases. The benchmarking suite was designed to provide an objective measure of the performance of these databases as well as to compare their capabilities for different types of data. This provides valuable insights into the suitability of different time series databases for different use cases and provides benchmarks that can be used to inform system design decisions.

==> plan.tex <==
The key objectives of this project are:\\
\begin{enumerate}
    \item Investigate current research on benchmarks for time series databases.
    \item Identify tasks frequently performed in the use case of high frequency trading data application to form a set of benchmarks.
    \item Implement the benchmarks in kdb+ and InfluxDB.
    \item Compare the performance of kdb+ and InfluxDB in terms of the benchmarks.
    \item Critically analyze the designed benchmarks and compare with existing benchmarks.
\end{enumerate}

The project begins with literature review and background study, which has been completed before the submission of this report. The Gantt chart below demonstrates the detailed project plan from June to the end of the project in early September. The software development and testing has been divided into two stages, where it will be implemented and tested on a local PC before the final testing on the university server. The software will be developed using the Agile method, which is suitable for smaller projects and faster delivery. Although literature review has already been performed before the implementation, it is also planned throughout the project for doing research on different parts of the project.
\\


\begin{enumerate}[label=\Alph*.]
    \item Implement kdb and InfluxDB data collection pipeline
    \item Collect data from crypto currency exchanges to use for testing
    \item use case study
    \item Implement benchmarks in kdb and InfluxDB
    \item Test benchmarks in kdb and InfluxDB on local PC
    \item Further implementation after initial testing
    \item Test benchmarks in kdb and InfluxDB on university server
    \item Literature review
    \item Comparison and analysis of test data
    \item Write dissertation (deadline 31 August 2022)
    \item Prepare presentation (deadline 5 to 9 September 2022)
\end{enumerate}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/gantt.eps} 
\caption{Project Plan Gantt Chart}
\end{figure}



==> tech.tex <==
\section{Data Collection}
This study uses data collected from cryptocurrency exchanges to simulate the data used in real world use cases. As cryptocurrency exchanges are implemented with blockchain, the trades performed on these exchanges are visible to everyone on the network. Real time trade data and historical trades data are easily accessible to users. Due to the distributed nature of blockchain, the data is also reliable and validated by the miners. The trades in cryptocurrency exchanges are identical to trades in real world exchanges besides the difference in the currency. Depending on the specific exchange, a cryptocurrency exchange could have a large volume of data stream that is similar the a real world exchange. These reasons make cryptocurrency exchange data ideal for simulating the data and work load of real world financial applications.
\\\\
Cryptofeed \parencite{cryptofeed} is used for collecting data from cryptocurrency exchanges in this project. It is an open source Python library designed for handling cryptocurrency exchange feeds. It can be used to retrieve real time or historical data. Cryptofeed can combine the feeds from an arbitrary combination of the supported exchanges into one standardized and normalized feed. Developers can register callbacks on events including trades, ticker updates to handle the data.


\begin{figure}[H]
\centering
\includegraphics[width=\columnwidth]{figures/kdb_collection_pipeline.eps} 
\caption{Kdb+ Data Collection Pipeline}
\label{kdb_collection_pipeline}
\end{figure}

Figure \ref{kdb_collection_pipeline} demonstrates the data collection pipeline using kdb+. Multiple exchanges generate their own data feeds from their operations. A FeedHandler is  defined in Cryptofeed to subscribe to feeds from specified exchanges and combined into one standardized feed where the data is transformed into Python objects.
\\\\
The callback for the unified feed generated by Cryptofeed is implemented with qPython. qPython \parencite{qPython} is a python library that enables communication between Python and kdb+/q processes. qPython first open on a connection with the kdb+ server, which has a q process listening on a specific port. When the data is received from feed subscription, Cryptofeed invoke the callback function which would preprocess the data, structure the query and send the data to the kdb+ server for storage.
\\\\
When the kdb+ server recieves the data on the open port, it first save the data in the Realtime Database in memory. Every day the content from the Realtime Database is persisted into the Historical Database on disk. Thus the Realtime Database can free up space to store incoming new data.


==> titlepage.tex <==
% Last modification: 2015-08-17 (Marc Deisenroth)
\begin{titlepage}

\newcommand{\HRule}{\rule{\linewidth}{0.5mm}} % Defines a new command for the horizontal lines, change thickness here


%----------------------------------------------------------------------------------------
%	LOGO SECTION
%----------------------------------------------------------------------------------------

\includegraphics[width = 4cm]{./figures/imperial}\\[0.5cm] 

\center % Center remainder of the page

%----------------------------------------------------------------------------------------
%	HEADING SECTIONS
%----------------------------------------------------------------------------------------

\textsc{\Large Imperial College London}\\[0.5cm] 
\textsc{\large Department of Computing}\\[0.5cm] 

%----------------------------------------------------------------------------------------
%	TITLE SECTION
%----------------------------------------------------------------------------------------

\HRule \\[0.4cm]
{ \huge \bfseries \reporttitle}\\ % Title of your document
\HRule \\[1.5cm]
 
%----------------------------------------------------------------------------------------
%	AUTHOR SECTION
%----------------------------------------------------------------------------------------

\begin{minipage}{0.4\textwidth}
\begin{flushleft} \large
\emph{Author:}\\
\reportauthor % Your name
\end{flushleft}
\end{minipage}
~
\begin{minipage}{0.4\textwidth}
\begin{flushright} \large
\emph{Supervisor:} \\
\supervisor % Supervisor's Name
\end{flushright}
\end{minipage}
\\[1cm]
\begin{minipage}{0.4\textwidth}
\begin{flushleft} \large
\emph{}\\
{} % Your name
\end{flushleft}
\end{minipage}
~
\begin{minipage}{0.4\textwidth}
\begin{flushright} \large
\emph{Second Marker:} \\
\secondmarker 
\end{flushright}
\end{minipage}



%----------------------------------------------------------------------------------------
%	FOOTER & DATE SECTION
%----------------------------------------------------------------------------------------
\vfill % Fill the rest of the page with whitespace
Submitted in partial fulfillment of the requirements for the MSc degree in
\degreetype~of Imperial College London\\[0.5cm]

\makeatletter
\@date 
\makeatother


\end{titlepage}

